LabVLA: Grounding Vision-Language-Action Models in Scientific Laboratories

Scientific laboratories increasingly rely on AI systems to reason about experiments, but the physical act of doing science remains largely outside their reach. AI can help read literature, generate hypotheses, and plan protocols, yet the execution of those protocols at the bench still requires a human operator. Vision-Language-Action (VLA) models provide one possible interface between written protocols and robot execution, but existing policies are trained mostly on household and tabletop demonstrations and rarely encounter the instruments, transparent liquids, or fixed protocol workflows found in scientific laboratories. Closing this gap requires both laboratory-specific supervision and a unified learning framework that can accommodate the diverse robot embodiments used to execute experimental protocols. We therefore identify data and embodiment as central bottlenecks alongside model design. To address the data side, we build RoboGenesis, a simulation-based workflow and data engine that composes configured laboratory workflows from atomic skills, validates and filters rollouts, and exports structured demonstrations across supported robot profiles. On the policy side, we present LabVLA, trained with a two-stage recipe: FAST action token pretraining first makes the Qwen3-VL-4B-Instruct backbone action aware before any continuous control is learned, and flow matching posttraining then attaches a DiT action expert under knowledge insulation. On the LabUtopia benchmark, LabVLA achieves the highest average success rate among all evaluated baselines under both in-distribution and out-of-distribution settings.

==> notations.tex <==
% \newcommand{\zdh}[1]{\textcolor{brown}{ZDH: #1}}
\newcommand{\yz}[1]{\textcolor{blue}{YZ: #1}}
% \newcommand{\rebuttal}[1]{{\color{blue}{#1}}}
% \newcommand{\rebuttal}[1]{{#1}}

\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\med}[1]{\textcolor{magenta}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}

\usepackage{xspace}
\newcommand*{\eg}{\textit{e.g.}\xspace}
\newcommand*{\ie}{\textit{i.e.}\xspace}
\newcommand*{\cf}{\textit{cf.}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
% \theoremstyle{remark}
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}


% modifed \bar{}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \newcommand{\refe}{\text{ref}} % \ref is used by latex default

\newcommand*{\dif}{\mathop{}\!\mathrm{d}}
% \newcommand{\KL}[2]{\mathcal{D}_{\mathrm{KL}}\left(#1\Vert #2\right)}
\newcommand{\tr}[1]{\text{tr}\left(#1\right)}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\def\viz{\emph{viz}\onedot}
\newcommand{\diag}[1]{\text{diag}\left(#1\right)}
\newcommand{\dt}{\frac{\dif}{\dif t}}

\newcommand{\aaa}{\mathbf{a}}
% \newcommand{\ccc}{\mathbf{c} % weird
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\s}{\mathbf{s}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\0}{\mathbf{0}}

\newcommand{\dd}{{\boldsymbol{\delta}}}
\newcommand{\eps}{{\boldsymbol{\epsilon}}}
\newcommand{\vtheta}{{\boldsymbol{\theta}}}
\newcommand{\vphi}{{\boldsymbol{\phi}}}
\newcommand{\ra}{{\rightarrow}}
\newcommand{\disteq}{{\stackrel{d}{=}}}

% \newcommand{\W}{\mathbf{W}}
% \newcommand{\Q}{\mathcal{Q}}
\newcommand{\A}{\mathcal{A}}
% \newcommand{\gB}{\mathcal{B}}
% \newcommand{\D}{\mathfrak{D}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\gE}{\mathcal{E}}
\newcommand{\LL}{{\mathcal{L}}}
\newcommand{\LDB}{\LL_{\text{DB}}}
\newcommand{\lDB}{\ell_{\text{DB}}}
\newcommand{\lFL}{\ell_{\text{FL}}}
\newcommand{\lFLDB}{\ell_{\text{FL-DB}}}
\newcommand{\lST}{\ell_{\text{SubTB}}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\gS}{\mathcal{S}}
% \newcommand{\Sm}{\Sigma}
% \newcommand{\La}{\Lambda}



% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
\def\TwoEqref#1#2{Equation \ref{#1} and \ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}

==> tables/analysis1.tex <==
\begin{table}[h]
\centering
\caption{Ablation study on LabUtopia tasks under in-distribution (ID) and out-of-distribution (OOD) settings.
Empty result cells indicate variants that are still in progress.}
\label{tab:analysis_training_ablation}
\vspace{-2mm}
\renewcommand{\arraystretch}{1.18}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{l c cccccc >{\centering\arraybackslash}p{3.2em}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Size}} & \multicolumn{6}{c}{\textbf{LabUtopia Tasks}} & \multirow{2}{*}{\textbf{Avg.}} \\
\cmidrule(lr){3-8}
 & & Pick Up & Press Button & Open Door & Pour Liquid & Heat Beaker & Transport Beaker & \\
\midrule
\multicolumn{9}{l}{\textit{In-Distribution}} \\[2pt]
\rowcolor{blue!6}
\textbf{LabVLA (Ours)} & 5B & \textbf{71.2} & 97.5 & \textbf{65.8} & 43.0 & 98.3 & 79.2 & \textbf{75.8} \\
No VLM pre-training & 5B &  &  &  &  &  &  &  \\
No LabEmbodied post-training & 5B &  &  &  &  &  &  &  \\
No knowledge insulation & 5B &  &  &  &  &  &  &  \\
Direct LabUtopia fine-tuning & 5B &  &  &  &  &  &  &  \\
\midrule
\multicolumn{9}{l}{\textit{Out-of-Distribution}} \\[2pt]
\rowcolor{blue!6}
\textbf{LabVLA (Ours)} & 5B & \textbf{64.2} & 98.3 & 65.0 & 30.8 & 95.0 & 85.0 & \textbf{73.1} \\
No VLM pre-training & 5B &  &  &  &  &  &  &  \\
No LabEmbodied post-training & 5B &  &  &  &  &  &  &  \\
No knowledge insulation & 5B &  &  &  &  &  &  &  \\
Direct LabUtopia fine-tuning & 5B &  &  &  &  &  &  &  \\
\bottomrule
\end{tabular}%
}
\end{table}




==> tables/analysis3.tex <==
\begin{table}[t]
\centering
\caption{Placeholder real-robot evaluation on a Franka laboratory setup.
Trial counts, success rates, and failure modes will be reported after hardware validation.}
\label{tab:analysis_franka}
\vspace{-2mm}
\renewcommand{\arraystretch}{1.12}
\resizebox{0.88\linewidth}{!}{%
\begin{tabular}{l c c l}
\toprule
\textbf{Task} & \textbf{Trials} & \textbf{Success Rate} & \textbf{Primary Failure Mode} \\
\midrule
Pick up labware & TBD & TBD & TBD \\
Press instrument button & TBD & TBD & TBD \\
Transfer container & TBD & TBD & TBD \\
Execute short laboratory protocol & TBD & TBD & TBD \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/main1.tex <==
% ==================== Level-4 长序列表格（暂未填充数据，保留备用） ====================
% \begin{table}[t]
% \centering
% \caption{Success rates (\%) on LabUtopia Level-4 long-horizon tasks.
% SP = single-stage primitive success rate; A1--A7 = sub-steps in the task sequence.}
% \label{tab:level4_results}
% \renewcommand{\arraystretch}{1.18}
% \resizebox{0.95\linewidth}{!}{%
% \begin{tabular}{l l c cccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Size}}
% & \multicolumn{8}{c}{\textbf{Success Rate (\%)}} \\
% \cmidrule(lr){4-11}
% & & & SP & A1 & A2 & A3 & A4 & A5 & A6 & A7 \\
% \midrule
% \multicolumn{11}{l}{\textit{Clean Beaker}} \\[2pt]
%  & ACT \cite{fu2024mobile}                         & $<$1B & 14.0 & 99.3 & 51.9 & 43.3 & 42.5 & 12.3 & 10.6 & 1.6 \\
%  & DP \cite{chi2025diffusion}                      & $<$1B & 2.5  & 92.7 & 8.1  & 1.3  & 0.0  & 0.0  & 0.0  & 0.0 \\
%  & SmolVLA \cite{shukor2025smolvla}                & $<$1B & --   & --   & --   & --   & --   & --   & --   & --  \\
%  & $\pi_0$ \cite{black2024pi_0}                    & 3B    & --   & --   & --   & --   & --   & --   & --   & --  \\
%  & $\pi_{0.5}$ \cite{intelligence2025pi_}          & 3B    & --   & --   & --   & --   & --   & --   & --   & --  \\
%  & \rowcolor{blue!6} \textbf{LabVLA (Ours)}        & 3B    & --   & --   & --   & --   & --   & --   & --   & --  \\
% \midrule
% \multicolumn{11}{l}{\textit{Drying Beakers}} \\[2pt]
%  & ACT \cite{fu2024mobile}                         & $<$1B & 6.3  & 81.3 & 42.0 & 19.7 & 9.3  & 3.5  & 1.2  & 0.0 \\
%  & DP \cite{chi2025diffusion}                      & $<$1B & 2.0  & 76.0 & 32.0 & 26.3 & 0.0  & 0.0  & 0.0  & 0.0 \\
%  & \rowcolor{blue!6} \textbf{LabVLA (Ours)}        & 3B    & --   & --   & --   & --   & --   & --   & --   & --  \\
% \midrule
% \multicolumn{11}{l}{\textit{Liquid Fusion}} \\[2pt]
%  & ACT \cite{fu2024mobile}                         & $<$1B & 8.3  & 96.3 & 57.6 & 46.7 & 42.5 & 12.3 & 10.6 & 1.6 \\
%  & DP \cite{chi2025diffusion}                      & $<$1B & 6.7  & 93.5 & 12.3 & 8.3  & 0.0  & 0.0  & 0.0  & 0.0 \\
%  & \rowcolor{blue!6} \textbf{LabVLA (Ours)}        & 3B    & --   & --   & --   & --   & --   & --   & --   & --  \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}


\begin{table}[t]
\centering
\caption{Success rates (\%) on AutoBio benchmark tasks across three difficulty levels.}
\label{tab:autobio_results}
\vspace{-2mm}
\small
\renewcommand{\arraystretch}{1.18}
% tabcolsep 控制列间距，可调整（默认6pt，增大则表格更宽）
\setlength{\tabcolsep}{8pt}
\begin{tabular}{l cccccc}
\toprule
\multirow{2}{*}{\textbf{Task}} & \multicolumn{6}{c}{\textbf{Success Rate (\%)}} \\
\cmidrule(lr){2-7}
 & SmolVLA & X-VLA & $\pi_0$ & $\pi_{0.5}$ & UniVLA & \textbf{LabVLA (Ours)} \\
\midrule
\multicolumn{7}{l}{\textit{Easy}} \\[2pt]
Close thermal cycler lid     & 100 & 99 & 100 & 100 & -- & -- \\
Open thermal cycler lid      &  97 & 100 &  98 &  95 & -- & -- \\
Pick up centrifuge tube      &  42 & 91 &  56 &  82 & -- & -- \\
\midrule
\multicolumn{7}{l}{\textit{Medium}} \\[2pt]
Unscrew centrifuge tube cap  &  19 & 0  &  17 &   8 & -- & -- \\
Aspirate with pipette        &  71 & 0  &  32 &  20 & -- & -- \\
Transfer centrifuge tube     &  26 & 7  &  44 &  36 & -- & -- \\
\midrule
\multicolumn{7}{l}{\textit{Hard}} \\[2pt]
Screw on centrifuge tube cap &   1 & 0  &   0 &   7 & -- & -- \\
Operate thermal mixer panel  &  0.2 & 0.3 &   5 &   0 & -- & -- \\
Load centrifuge rotor        &  16 & 3  &   9 &  13 & -- & -- \\
\bottomrule
\end{tabular}
\end{table}





















